Applications and Challenges of Sentiment Analysis in Real-life Scenarios

Sentiment analysis has benefited from the availability of lexicons and benchmark datasets created over decades of research. However, its applications to the real world are a driving force for research in SA. This chapter describes some of these applications and related challenges in real-life scenarios. In this chapter, we focus on five applications of SA: health, social policy, e-commerce, digital humanities and other areas of NLP. This chapter is intended to equip an NLP researcher with the `what', `why' and `how' of applications of SA: what is the application about, why it is important and challenging and how current research in SA deals with the application. We note that, while the use of deep learning techniques is a popular paradigm that spans these applications, challenges around privacy and selection bias of datasets is a recurring theme across several applications.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter1.tex <==
\begin{frontmatter}

\chapter{Chapter Title}\label{chap1}
\subchapter{Chapter Subtitle}

% \minitoc

\begin{abstract}
 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.
\end{abstract}

\begin{keywords}
\kwd{One}
\kwd{Two}
\kwd{Three}
\end{keywords}

\end{frontmatter}


\section{Section title}\label{sec1}

% \begin{figure}
% \title{}% Figure title
% \caption{}% Figure caption
% \label{}%
% \end{figure}

% \begin{table}
% \title{}% Table title
% \caption{}% Table caption
% \label{}%
% \end{table}



==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...


==> preface.tex <==
\cleardoublepage
\begin{frontmatter}
\chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
\end{frontmatter}


 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

\source%
{%
  \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
}


==> references.tex <==
%\begin{frontmatter}
%  \chapter*{References}
%  \markboth{References}{References}
%\end{frontmatter}

\begin{thebibliography}{10}

% \bibitem{..}
% \bibitem[]{..}

\end{thebibliography}

==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    \title{Book title}
    %\subtitle{Book Subtitle}
    %\volume{2}
  \end{titlepagerule}

  \edition{2nd edition}

%  \editedby{Edited by}

  \author{Author Firstname  Surname}
  \address{Author Address\\Department of Chemistry\\University of Florida}

  \author{Author Firstname  Surname}
  \address{Author Address}
\end{titlepage}

